The Cluster HEritage project with XMM-Newton: Mass Assembly and Thermodynamics at the Endpoint of structure formation. I. Programme overview

The Cluster HEritage project with XMM-Newton - Mass Assembly and Thermodynamics at the Endpoint of structure formation (CHEX-MATE) is a three mega-second Multi-Year Heritage Programme to obtain X-ray observations of a minimally-biased, signal-to-noise limited sample of 118 galaxy clusters detected by Planck through the Sunyaev-Zeldovich effect. The programme, described in detail in this paper, aims to study the ultimate products of structure formation in time and mass. It is composed of a census of the most recent objects to have formed (Tier-1: 0.05 < z < 0.2; 2 x 10e14 M_sun < M_500 < 9 x 10e14 M_sun), together with a sample of the highest-mass objects in the Universe (Tier-2: z < 0.6; M_500 > 7.25 x 10e14 M_sun). The programme will yield an accurate vision of the statistical properties of the underlying population, measure how the gas properties are shaped by collapse into the dark matter halo, uncover the provenance of non-gravitational heating, and resolve the major uncertainties in mass determination that limit the use of clusters for cosmological parameter estimation. We will acquire X-ray exposures of uniform depth, designed to obtain individual mass measurements accurate to 15-20% under the hydrostatic assumption. We present the project motivations, describe the programme definition, and detail the ongoing multi-wavelength observational (lensing, SZ, radio) and theoretical effort that is being deployed in support of the project.

==> master_2.tex <==
 Name & RA    & Dec  & $z$ & $M_{500}$ & SNR & Tier & $n_H$ & $t_{\rm XMM}$ & $t_{\rm CXO}$ & $t_{\rm XMM, new}$ \\
      & h:m:s & d:m:s &    & $10^{14} M_{\odot}$ & & & $10^{20}$ cm$^{-2}$ & ksec & ksec & ksec \\ \hline 
PSZ2 G111.75+70.37 & 13:13:06.4 & +46:16:51 & 0.1830 & 4.3 & 8.3 & 1 & 1.1 & 0.0 & 0.0 & 36.0 \\
PSZ2 G113.29-29.69 & 00:11:45.9 & +32:24:51 & 0.1073 & 3.6 & 8.1 & 1 & 4.7 & 0.0 & 8.1 & 21.0 \\
PSZ2 G113.91-37.01 & 00:19:41.7 & +25:18:05 & 0.3712 & 7.6 & 8.2 & 2 & 2.9 & 0.0 & 0.0 & 49.0 \\
PSZ2 G114.79-33.71 & 00:20:37.5 & +28:39:32 & 0.0940 & 3.8 & 9.4 & 1 & 3.9 & 0.0 & 14.1 & 21.0 \\
PSZ2 G124.20-36.48 & 00:55:50.6 & +26:24:36 & 0.1971 & 7.3 & 12.8 & 12 & 5.4 & 40.7 & 366.3 & 0.0 \\
PSZ2 G143.26+65.24 & 11:59:14.8 & +49:47:33 & 0.3634 & 7.3 & 10.2 & 2 & 2.2 & 0.0 & 22.1 & 45.0 \\
PSZ2 G149.39-36.84 & 02:21:33.6 & +21:21:42 & 0.1700 & 5.3 & 7.3 & 1 & 7.5 & 0.0 & 0.0 & 28.0 \\
PSZ2 G155.27-68.42 & 01:37:24.8 & -08:27:20 & 0.5670 & 8.4 & 8.0 & 2 & 3.5 & 24.9 & 0.0 & 51.0 \\
PSZ2 G159.91-73.50 & 01:31:52.6 & -13:36:43 & 0.2060 & 8.5 & 17.1 & 2 & 1.4 & 63.7 & 20.2 & 0.0 \\
PSZ2 G172.74+65.30 & 11:11:40.4 & +40:50:14 & 0.0794 & 2.4 & 7.5 & 1 & 1.3 & 0.0 & 11.7 & 23.0 \\
PSZ2 G172.98-53.55 & 02:39:53.3 & -01:34:44 & 0.3730 & 7.4 & 7.6 & 2 & 3.0 & 130.0 & 96.3 & 0.0 \\
PSZ2 G179.09+60.12 & 10:40:44.5 & +39:57:11 & 0.1372 & 3.8 & 7.5 & 1 & 1.7 & 36.6 & 58.1 & 27.0 \\
PSZ2 G186.37+37.26 & 08:42:57.2 & +36:22:03 & 0.2820 & 11.0 & 18.9 & 2 & 2.9 & 22.4 & 27.9 & 21.0 \\
PSZ2 G187.53+21.92 & 07:32:20.4 & +31:37:59 & 0.1710 & 5.2 & 8.1 & 1 & 4.9 & 18.6 & 217.6 & 21.0 \\
PSZ2 G192.18+56.12 & 10:16:21.9 & +33:38:26 & 0.1240 & 3.6 & 7.8 & 1 & 1.5 & 0.0 & 5.1 & 25.0 \\
PSZ2 G195.75-24.32 & 04:54:06.5 & +02:54:25 & 0.2030 & 7.8 & 11.8 & 2 & 5.7 & 42.4 & 535.2 & 0.0 \\
PSZ2 G201.50-27.31 & 04:54:11.1 & -03:00:58 & 0.5377 & 8.3 & 7.1 & 2 & 3.9 & 42.6 & 58.8 & 56.0 \\
PSZ2 G204.10+16.51 & 07:35:47.5 & +15:06:48 & 0.1220 & 3.7 & 6.7 & 1 & 5.0 & 0.0 & 0.0 & 28.0 \\
PSZ2 G205.93-39.46 & 04:17:34.1 & -11:54:18 & 0.4430 & 11.5 & 13.8 & 2 & 3.3 & 0.0 & 90.3 & 26.0 \\
PSZ2 G206.45+13.89 & 07:29:50.7 & +11:56:28 & 0.4100 & 7.5 & 7.3 & 2 & 5.8 & 25.0 & 0.0 & 51.0 \\
PSZ2 G207.88+81.31 & 12:12:18.2 & +27:33:05 & 0.3530 & 7.4 & 10.1 & 2 & 1.7 & 0.0 & 14.8 & 43.0 \\
PSZ2 G208.80-30.67 & 04:54:06.7 & -10:13:08 & 0.2475 & 7.3 & 9.5 & 2 & 4.8 & 85.5 & 168.6 & 0.0 \\
PSZ2 G210.64+17.09 & 07:48:46.6 & +09:40:00 & 0.4800 & 7.8 & 7.6 & 2 & 2.7 & 11.7 & 0.0 & 60.0 \\
PSZ2 G216.62+47.00 & 09:49:51.5 & +17:07:09 & 0.3826 & 8.5 & 9.8 & 2 & 3.1 & 12.7 & 35.6 & 43.0 \\
PSZ2 G217.09+40.15 & 09:24:05.9 & +14:10:26 & 0.1357 & 3.9 & 7.0 & 1 & 3.3 & 0.0 & 30.1 & 28.0 \\
PSZ2 G217.40+10.88 & 07:38:18.4 & +01:02:15 & 0.1890 & 5.3 & 7.8 & 1 & 8.5 & 0.0 & 0.0 & 37.0 \\
PSZ2 G218.59+71.31 & 11:29:54.5 & +23:48:14 & 0.1371 & 3.8 & 7.2 & 1 & 1.2 & 0.0 & 0.0 & 30.0 \\
PSZ2 G218.81+35.51 & 09:09:12.6 & +10:58:32 & 0.1751 & 5.2 & 8.4 & 1 & 3.2 & 27.4 & 34.9 & 21.0 \\
PSZ2 G224.00+69.33 & 11:23:57.6 & +21:28:56 & 0.1904 & 5.1 & 8.8 & 1 & 1.6 & 0.0 & 20.1 & 27.0 \\
PSZ2 G225.93-19.99 & 06:00:08.1 & -20:08:07 & 0.4350 & 9.8 & 12.4 & 2 & 4.9 & 9.0 & 0.0 & 26.0 \\
PSZ2 G226.18+76.79 & 11:55:17.9 & +23:24:18 & 0.1427 & 6.0 & 14.6 & 1 & 1.8 & 279.8 & 157.9 & 0.0 \\
PSZ2 G228.16+75.20 & 11:49:35.1 & +22:24:08 & 0.5450 & 9.8 & 11.4 & 2 & 1.9 & 24.7 & 370.2 & 42.0 \\
PSZ2 G229.74+77.96 & 12:01:13.2 & +23:06:21 & 0.2690 & 7.4 & 12.0 & 2 & 2.2 & 0.0 & 26.1 & 27.0 \\
PSZ2 G238.69+63.26 & 11:12:54.3 & +13:26:05 & 0.1690 & 4.2 & 7.3 & 1 & 1.6 & 50.0 & 93.2 & 0.0 \\
PSZ2 G239.27-26.01 & 05:53:28.4 & -33:42:33 & 0.4300 & 8.8 & 12.2 & 2 & 3.3 & 0.0 & 85.1 & 49.0 \\
PSZ2 G241.11-28.68 & 05:42:57.1 & -35:59:49 & 0.4200 & 7.4 & 9.0 & 2 & 3.0 & 10.0 & 0.0 & 55.0 \\
PSZ2 G243.15-73.84 & 01:59:02.7 & -34:12:57 & 0.4100 & 8.1 & 10.3 & 2 & 1.5 & 0.0 & 19.5 & 48.0 \\
PSZ2 G243.64+67.74 & 11:32:51.9 & +14:27:11 & 0.0834 & 3.6 & 12.0 & 1 & 2.9 & 0.0 & 9.1 & 21.0 \\
PSZ2 G259.98-63.43 & 02:32:18.7 & -44:20:46 & 0.2836 & 7.5 & 13.0 & 2 & 1.7 & 10.0 & 23.7 & 21.0 \\
PSZ2 G262.27-35.38 & 05:16:37.4 & -54:30:10 & 0.2952 & 8.8 & 22.9 & 2 & 2.1 & 58.1 & 31.4 & 0.0 \\
PSZ2 G262.73-40.92 & 04:38:17.4 & -54:19:23 & 0.4210 & 7.5 & 12.7 & 2 & 1.0 & 14.7 & 20.0 & 42.0 \\
PSZ2 G263.68-22.55 & 06:45:28.8 & -54:13:37 & 0.1644 & 8.0 & 21.7 & 2 & 5.6 & 47.4 & 10.1 & 0.0 \\
PSZ2 G266.04-21.25 & 06:58:30.0 & -55:56:23 & 0.2965 & 12.5 & 28.4 & 2 & 4.9 & 38.7 & 584.2 & 0.0 \\
PSZ2 G266.83+25.08 & 10:23:50.2 & -27:15:21 & 0.2542 & 7.3 & 11.7 & 2 & 5.6 & 0.0 & 37.2 & 29.0 \\
PSZ2 G271.18-30.95 & 05:49:19.6 & -62:05:13 & 0.3700 & 7.4 & 14.1 & 2 & 4.5 & 10.0 & 0.0 & 46.0 \\
PSZ2 G273.59+63.27 & 12:00:25.4 & +03:20:49 & 0.1339 & 5.5 & 12.6 & 1 & 2.1 & 14.7 & 19.6 & 21.0 \\
PSZ2 G277.76-51.74 & 02:54:16.1 & -58:56:52 & 0.4380 & 8.7 & 15.1 & 2 & 1.9 & 68.6 & 0.0 & 0.0 \\
PSZ2 G278.58+39.16 & 11:31:54.2 & -19:55:40 & 0.3075 & 8.3 & 12.2 & 2 & 4.0 & 10.0 & 99.2 & 21.0 \\
PSZ2 G283.91+73.87 & 10:16:21.9 & +33:38:26 & 0.0852 & 2.7 & 8.4 & 1 & 2.1 & 0.0 & 42.0 & 21.0 \\
PSZ2 G284.41+52.45 & 12:06:12.0 & -08:48:03 & 0.4414 & 10.4 & 13.6 & 2 & 4.3 & 178.9 & 203.8 & 0.0 \\
PSZ2 G285.63+72.75 & 12:30:47.6 & +10:33:11 & 0.1650 & 5.6 & 10.9 & 1 & 2.1 & 0.0 & 19.2 & 21.0 \\
PSZ2 G286.98+32.90 & 11:50:49.0 & -28:04:28 & 0.3900 & 13.7 & 22.7 & 2 & 7.3 & 10.0 & 199.0 & 21.0 \\
PSZ2 G287.46+81.12 & 12:41:17.6 & +18:34:28 & 0.0730 & 2.6 & 7.4 & 1 & 1.5 & 15.5 & 0.0 & 0.0 \\
PSZ2 G313.33+61.13 & 13:11:29.3 & -01:20:27 & 0.1832 & 8.8 & 16.7 & 2 & 1.8 & 84.8 & 199.8 & 0.0 \\
PSZ2 G313.88-17.11 & 16:01:49.2 & -75:45:14 & 0.1530 & 7.9 & 16.6 & 2 & 5.9 & 31.5 & 9.1 & 0.0 \\
PSZ2 G324.04+48.79 & 13:47:30.5 & -11:45:07 & 0.4516 & 10.6 & 11.5 & 2 & 4.6 & 36.5 & 335.5 & 0.0 \\
PSZ2 G325.70+17.34 & 14:47:33.9 & -40:20:38 & 0.3155 & 7.6 & 8.7 & 2 & 6.8 & 0.0 & 30.1 & 45.0 \\
PSZ2 G339.63-69.34 & 23:44:43.9 & -42:43:11 & 0.5960 & 8.1 & 9.2 & 2 & 1.5 & 237.2 & 558.7 & 0.0 \\
PSZ2 G340.36+60.58 & 14:01:02.2 & +02:52:43 & 0.2528 & 9.2 & 15.6 & 2 & 2.0 & 368.4 & 363.7 & 0.0 \\
PSZ2 G340.94+35.07 & 14:59:29.0 & -18:10:44 & 0.2357 & 7.8 & 10.5 & 2 & 7.4 & 0.0 & 40.2 & 24.0 \\
PSZ2 G346.61+35.06 & 15:15:03.1 & -15:22:46 & 0.2226 & 8.4 & 12.9 & 2 & 8.3 & 0.0 & 60.0 & 21.0 \\
PSZ2 G349.46-59.95 & 22:48:44.4 & -44:31:58 & 0.3475 & 11.4 & 20.7 & 2 & 1.2 & 39.8 & 125.2 & 0.0 \\


==> tab_lensing_data_1.tex <==
Name              	 & 	SuP@Subaru       	 & 	HSC@Subaru	 & 	 Megacam@CFHT 	 & 	OC@VST   	 & 	HAWKI	 & 	WFI@MPG/ESO                                             	 & 	WL samples            	 & 	WL surveys  	\\
\midrule
PSZ2 G075.71+13.51	 & 	$B_J V_J R_C i^+$	 & 	$i^+$     	 & 	$g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G068.22+15.18	 & 	--               	 & 	--        	 & 	$r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G040.03+74.95	 & 	--               	 & 	--        	 & 	$r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G033.81+77.18	 & 	--               	 & 	--        	 & 	$g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,CCCP100           	 & 	--          	\\
PSZ2 G057.78+52.32	 & 	--               	 & 	--        	 & 	 -- 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	CFIS        	\\
PSZ2 G105.55+77.21	 & 	--               	 & 	$i^+$     	 & 	$u g i$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	CFIS        	\\
PSZ2 G042.81+56.61	 & 	--               	 & 	$i^+$     	 & 	$g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,CCCP100           	 & 	--          	\\
PSZ2 G031.93+78.71	 & 	--               	 & 	--        	 & 	$r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G287.46+81.12	 & 	--               	 & 	--        	 & 	$r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G040.58+77.12	 & 	--               	 & 	--        	 & 	$r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G057.92+27.64	 & 	--               	 & 	--        	 & 	 -- 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	CFIS        	\\
PSZ2 G006.49+50.56	 & 	--               	 & 	--        	 & 	$g r i$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,PSZ2LS,CCCP100    	 & 	RCSLS       	\\
PSZ2 G048.10+57.16	 & 	$g^+ r^+ i^+$    	 & 	--        	 & 	$u g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	CFIS        	\\
PSZ2 G172.74+65.30	 & 	--               	 & 	--        	 & 	 -- 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	CFIS        	\\
PSZ2 G057.61+34.93	 & 	--               	 & 	--        	 & 	$u g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	CFIS        	\\
PSZ2 G243.64+67.74	 & 	--               	 & 	--        	 & 	$r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G283.91+73.87	 & 	--               	 & 	--        	 & 	$u g r i$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G080.16+57.65	 & 	--               	 & 	--        	 & 	 -- 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	CFIS        	\\
PSZ2 G044.20+48.66	 & 	$g^+ R_C$        	 & 	--        	 & 	$g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,CCCP100           	 & 	--          	\\
PSZ2 G028.63+50.15	 & 	--               	 & 	--        	 & 	$r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G114.79-33.71	 & 	--               	 & 	--        	 & 	$g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,CCCP100           	 & 	--          	\\
PSZ2 G056.77+36.32	 & 	--               	 & 	--        	 & 	 -- 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2                   	 & 	CFIS        	\\
PSZ2 G049.32+44.37	 & 	--               	 & 	--        	 & 	$g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G080.37+14.64	 & 	--               	 & 	--        	 & 	$r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G099.48+55.60	 & 	--               	 & 	--        	 & 	$u g r i$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,PSZ2LS            	 & 	CFIS,CFHTLS 	\\
PSZ2 G080.41-33.24	 & 	--               	 & 	--        	 & 	$g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,CCCP100           	 & 	--          	\\
PSZ2 G113.29-29.69	 & 	--               	 & 	--        	 & 	$g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,CCCP100           	 & 	CFIS        	\\
PSZ2 G053.53+59.52	 & 	$B_J g^+ R_C z^+$	 & 	--        	 & 	 -- 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2                   	 & 	CFIS        	\\
PSZ2 G046.88+56.48	 & 	$V_J R_C i^+$    	 & 	--        	 & 	$g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,CCCP100           	 & 	--          	\\
PSZ2 G204.10+16.51	 & 	--               	 & 	--        	 & 	$u r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G192.18+56.12	 & 	--               	 & 	--        	 & 	$g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,CCCP100           	 & 	CFIS        	\\
PSZ2 G098.44+56.59	 & 	--               	 & 	--        	 & 	$u g r i$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,PSZ2LS            	 & 	CFIS        	\\
PSZ2 G273.59+63.27	 & 	--               	 & 	--        	 & 	 -- 	 & 	$r^+ i^+$	 & 	--   	 & 	$B_{J,842} V_{843} R_{C,844}$                           	 & 	LC2                   	 & 	HSC-SSP,KiDS	\\
PSZ2 G217.09+40.15	 & 	--               	 & 	$i^+$     	 & 	$u g r i$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,CCCP100           	 & 	--          	\\
PSZ2 G218.59+71.31	 & 	--               	 & 	$i^+$     	 & 	 -- 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G179.09+60.12	 & 	--               	 & 	--        	 & 	$g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,CCCP100           	 & 	CFIS        	\\
PSZ2 G226.18+76.79	 & 	$B_J V_J R_C i^+$	 & 	--        	 & 	$u g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,CCCP100           	 & 	--          	\\
PSZ2 G077.90-26.63	 & 	$V_J i^+$        	 & 	--        	 & 	$g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G021.10+33.24	 & 	$V_J i^+$        	 & 	--        	 & 	$g r$ 	 & 	--       	 & 	--   	 & 	$B_{J,842} R_{C,844} I_{C,879}$                         	 & 	LC2,LoCuSS,WtG,CCCP100	 & 	--          	\\
PSZ2 G313.88-17.11	 & 	--               	 & 	--        	 & 	 -- 	 & 	$r^+$    	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G028.89+60.13	 & 	$V_J R_C i^+$    	 & 	--        	 & 	 -- 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,LoCuSS            	 & 	--          	\\
PSZ2 G071.63+29.78	 & 	--               	 & 	--        	 & 	 -- 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	CFIS        	\\
PSZ2 G062.46-21.35	 & 	--               	 & 	--        	 & 	$r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G094.69+26.36	 & 	--               	 & 	--        	 & 	 -- 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	CFIS        	\\
PSZ2 G066.68+68.44	 & 	$V_J i^+$        	 & 	--        	 & 	$i$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	CFIS        	\\
PSZ2 G050.40+31.17	 & 	$V_J i^+$        	 & 	--        	 & 	$g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,CCCP100           	 & 	--          	\\
PSZ2 G049.22+30.87	 & 	$V_J R_C$        	 & 	--        	 & 	 -- 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,LoCuSS,WtG        	 & 	--          	\\
PSZ2 G263.68-22.55	 & 	--               	 & 	--        	 & 	 -- 	 & 	$r^+$    	 & 	--   	 & 	$B_{J,841} B_{99} B_{J,878} V_{843} R_{C,844} I_{C,879}$	 & 	LC2                   	 & 	DES         	\\
PSZ2 G285.63+72.75	 & 	$V_J i^+$        	 & 	--        	 & 	$u g r i$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2                   	 & 	--          	\\
PSZ2 G238.69+63.26	 & 	$V_J i^+$        	 & 	--        	 & 	 -- 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G149.39-36.84	 & 	--               	 & 	--        	 & 	$r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G000.13+78.04	 & 	--               	 & 	--        	 & 	 -- 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G187.53+21.92	 & 	$V_J i^+$        	 & 	--        	 & 	$g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,LoCuSS,CCCP100    	 & 	--          	\\
PSZ2 G067.17+67.46	 & 	$g^+ V_J R_C i^+$	 & 	--        	 & 	$g r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,LoCuSS,CCCP100    	 & 	CFIS        	\\
PSZ2 G218.81+35.51	 & 	$V_J R_C i^+$    	 & 	--        	 & 	 -- 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	LC2,LoCuSS,WtG,CCCP100	 & 	--          	\\
PSZ2 G067.52+34.75	 & 	--               	 & 	--        	 & 	 -- 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	CFIS        	\\
PSZ2 G041.45+29.10	 & 	$V_J i^+$        	 & 	--        	 & 	 -- 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	--          	\\
PSZ2 G085.98+26.69	 & 	--               	 & 	--        	 & 	$r$ 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	CFIS        	\\
PSZ2 G111.75+70.37	 & 	--               	 & 	--        	 & 	 -- 	 & 	--       	 & 	--   	 & 	--                                                      	 & 	--                    	 & 	CFIS        	\\


==> tab_lensing_data_2.tex <==
Name              	 & 	SuP@Subaru                 	 & 	HSC@Subaru     	 & 	 Megacam@CFHT 	 & 	OC@VST       	 & 	HAWKI    	 & 	WFI@MPG/ESO                                                              	 & 	WL samples                     	 & 	WL surveys       	\\
\midrule
PSZ2 G313.33+61.13	 & 	$B_J V_J R_C i^+ z^+$      	 & 	--             	 & 	 -- 	 & 	$r^+ i^+$    	 & 	$J K_S$  	 & 	$B_{99} B_{J,878} V_{843} R_{C,844} R_{C,162} I_{C,879}$                 	 & 	LC2,LoCuSS                     	 & 	HSC-SSP,KiDS     	\\
PSZ2 G083.86+85.09	 & 	$V_J$                      	 & 	--             	 & 	 -- 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	CFIS             	\\
PSZ2 G217.40+10.88	 & 	--                         	 & 	--             	 & 	$r$ 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	--               	\\
PSZ2 G224.00+69.33	 & 	$V_J i^+$                  	 & 	--             	 & 	$g r$ 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	LC2,CCCP100                    	 & 	--               	\\
PSZ2 G124.20-36.48	 & 	$V_J i^+$                  	 & 	--             	 & 	$g r$ 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	LC2,LoCuSS,CCCP100             	 & 	--               	\\
PSZ2 G195.75-24.32	 & 	$V_J R_C i^+$              	 & 	--             	 & 	$g r$ 	 & 	--           	 & 	--       	 & 	$B_{99} V_{89} R_{C,844}$                                                	 & 	LC2,CCCP100                    	 & 	--               	\\
PSZ2 G159.91-73.50	 & 	$B_J V_J R_C i^+ z^+$      	 & 	--             	 & 	 -- 	 & 	$r^+$        	 & 	--       	 & 	$B_{J,878} V_{843} I_{C,879}$                                            	 & 	LC2,CLASH-WL,LoCuSS,WtG,CCCP100	 & 	DES              	\\
PSZ2 G346.61+35.06	 & 	--                         	 & 	$i^+$          	 & 	 -- 	 & 	$g^+ r^+ i^+$	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	--               	\\
PSZ2 G055.59+31.85	 & 	$V_J R_C i^+$              	 & 	--             	 & 	$u g r$ 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	LC2,CLASH-WL,LoCuSS,WtG,CCCP100	 & 	CFIS             	\\
PSZ2 G092.71+73.46	 & 	$V_J i^+$                  	 & 	--             	 & 	 -- 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	LC2,LoCuSS,CCCP100             	 & 	CFIS             	\\
PSZ2 G072.62+41.46	 & 	$B_J V_J R_C i^+$          	 & 	--             	 & 	 -- 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	LC2,LoCuSS,WtG,CCCP100         	 & 	CFIS             	\\
PSZ2 G073.97-27.82	 & 	$B_J V_J R_C i^+ I_C z^+$  	 & 	--             	 & 	$u$ 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	LC2,LoCuSS,WtG,CCCP100         	 & 	--               	\\
PSZ2 G340.94+35.07	 & 	--                         	 & 	--             	 & 	$i$ 	 & 	$r^+$        	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	--               	\\
PSZ2 G208.80-30.67	 & 	$V_J R_C i^+ z^+$          	 & 	--             	 & 	$g r$ 	 & 	$r^+$        	 & 	--       	 & 	--                                                                       	 & 	LC2,LoCuSS,WtG,CCCP100         	 & 	--               	\\
PSZ2 G340.36+60.58	 & 	$I_C$                      	 & 	--             	 & 	$g r$ 	 & 	$r^+ i^+$    	 & 	--       	 & 	$B_{J,878} V_{843}$                                                      	 & 	LC2,LoCuSS,WtG,CCCP100         	 & 	HSC-SSP,KiDS     	\\
PSZ2 G266.83+25.08	 & 	--                         	 & 	$i^+$          	 & 	 -- 	 & 	$r^+$        	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	--               	\\
PSZ2 G229.74+77.96	 & 	--                         	 & 	$i^+$          	 & 	 -- 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	--               	\\
PSZ2 G087.03-57.37	 & 	$B_J V_J R_C i^+$          	 & 	--             	 & 	$r i$ 	 & 	--           	 & 	--       	 & 	$B_{J,842} V_{843} R_{C,844}$                                            	 & 	LC2,PSZ2LS,LoCuSS,WtG          	 & 	HSC-SSP,RCSLS,DES	\\
PSZ2 G107.10+65.32	 & 	$B_J g^+ V_J R_C i^+ z^+$  	 & 	--             	 & 	$g r$ 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	LC2,LoCuSS,WtG,CCCP100         	 & 	CFIS             	\\
PSZ2 G186.37+37.26	 & 	$V_J i^+$                  	 & 	--             	 & 	$g r$ 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	LC2,LoCuSS,CCCP100             	 & 	CFIS             	\\
PSZ2 G259.98-63.43	 & 	--                         	 & 	--             	 & 	 -- 	 & 	$r^+ i^+$    	 & 	--       	 & 	$B_{99} B_{J,878} V_{843} V_{89} R_{C,844} R_{C,162} I_{C,879}$          	 & 	LC2                            	 & 	DES              	\\
PSZ2 G106.87-83.23	 & 	$V_J i^+$                  	 & 	--             	 & 	 -- 	 & 	--           	 & 	--       	 & 	$B_{J,842} B_{J,878} V_{843} R_{C,844}$                                  	 & 	LC2,LoCuSS                     	 & 	DES              	\\
PSZ2 G262.27-35.38	 & 	--                         	 & 	--             	 & 	 -- 	 & 	$r^+$        	 & 	--       	 & 	$B_{J,842} B_{J,878} V_{843} R_{C,844} I_{C,879}$                        	 & 	LC2                            	 & 	DES              	\\
PSZ2 G266.04-21.25	 & 	--                         	 & 	--             	 & 	 -- 	 & 	$r^+$        	 & 	$J K_S$  	 & 	$B_{J,842} B_{J,878} V_{843} R_{C,844} I_{C,845}$                        	 & 	LC2                            	 & 	DES              	\\
PSZ2 G008.94-81.22	 & 	$B_J R_C i^+ z^+$          	 & 	--             	 & 	$i$ 	 & 	$r^+ i^+$    	 & 	$K_S$    	 & 	$B_{99} B_{J,842} V_{843} V_{89} R_{C,844} R_{C,162} I_{C,879} z^{+,846}$	 & 	LC2                            	 & 	KiDS,DES         	\\
PSZ2 G278.58+39.16	 & 	$g^+ r^+$                  	 & 	--             	 & 	$r$ 	 & 	$i^+$        	 & 	--       	 & 	$B_{J,842} B_{J,878} V_{843} R_{C,844}$                                  	 & 	LC2                            	 & 	--               	\\
PSZ2 G008.31-64.74	 & 	--                         	 & 	--             	 & 	 -- 	 & 	$r^+ i^+$    	 & 	$J$      	 & 	--                                                                       	 & 	--                             	 & 	KiDS             	\\
PSZ2 G325.70+17.34	 & 	--                         	 & 	--             	 & 	 -- 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	--               	\\
PSZ2 G349.46-59.95	 & 	--                         	 & 	--             	 & 	 -- 	 & 	$g^+ r^+ i^+$	 & 	$K_S$    	 & 	$B_{J,842} V_{843} R_{C,844} I_{C,879} z^{+,846}$                        	 & 	LC2,CLASH-WL                   	 & 	DES              	\\
PSZ2 G207.88+81.31	 & 	--                         	 & 	--             	 & 	$r i$ 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	--               	\\
PSZ2 G143.26+65.24	 & 	--                         	 & 	$i^+$          	 & 	$r$ 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	CFIS             	\\
PSZ2 G271.18-30.95	 & 	--                         	 & 	--             	 & 	 -- 	 & 	$r^+$        	 & 	$K_S$    	 & 	--                                                                       	 & 	--                             	 & 	DES              	\\
PSZ2 G113.91-37.01	 & 	--                         	 & 	--             	 & 	 -- 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	--               	\\
PSZ2 G172.98-53.55	 & 	$B_J V_J R_C i^+ I_C z^+ Y$	 & 	$z^+ Y$        	 & 	$u g r i$ 	 & 	--           	 & 	$J K_S$  	 & 	$R_{C,844} I_{C,879}$                                                    	 & 	LC2,WtG,CCCP100                	 & 	HSC-SSP,DES      	\\
PSZ2 G216.62+47.00	 & 	$B_J V_J R_C i^+ I_C z^+$  	 & 	$i^+$          	 & 	$u$ 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	LC2,WtG                        	 & 	--               	\\
PSZ2 G046.10+27.18	 & 	$B_J V_J R_C I_C z^+$      	 & 	--             	 & 	$u r$ 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	LC2,WtG                        	 & 	--               	\\
PSZ2 G286.98+32.90	 & 	$g^+ r^+$                  	 & 	--             	 & 	$g$ 	 & 	$g^+ i^+$    	 & 	$K_S$    	 & 	$V_{843} R_{C,844} I_{C,879}$                                            	 & 	LC2                            	 & 	--               	\\
PSZ2 G057.25-45.34	 & 	$B_J V_J R_C i^+ I_C z^+$  	 & 	--             	 & 	$u r$ 	 & 	$r^+$        	 & 	--       	 & 	--                                                                       	 & 	LC2,WtG                        	 & 	--               	\\
PSZ2 G243.15-73.84	 & 	--                         	 & 	--             	 & 	 -- 	 & 	$r^+ i^+$    	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	KiDS,DES         	\\
PSZ2 G206.45+13.89	 & 	--                         	 & 	--             	 & 	$u r$ 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	--               	\\
PSZ2 G083.29-31.03	 & 	$B_J R_C I_C z^+$          	 & 	--             	 & 	$u g r i$ 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	LC2,WtG                        	 & 	--               	\\
PSZ2 G241.11-28.68	 & 	--                         	 & 	--             	 & 	 -- 	 & 	$r^+$        	 & 	--       	 & 	$R_{C,844}$                                                              	 & 	--                             	 & 	DES              	\\
PSZ2 G262.73-40.92	 & 	--                         	 & 	--             	 & 	 -- 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	DES              	\\
PSZ2 G239.27-26.01	 & 	--                         	 & 	--             	 & 	 -- 	 & 	$r^+ i^+$    	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	DES              	\\
PSZ2 G225.93-19.99	 & 	--                         	 & 	$r^+ i^+$      	 & 	 -- 	 & 	--           	 & 	$K_S$    	 & 	--                                                                       	 & 	--                             	 & 	--               	\\
PSZ2 G277.76-51.74	 & 	--                         	 & 	--             	 & 	 -- 	 & 	--           	 & 	--       	 & 	$R_{C,844}$                                                              	 & 	--                             	 & 	DES              	\\
PSZ2 G284.41+52.45	 & 	$B_J V_J R_C I_C z^+$      	 & 	--             	 & 	$g r i$ 	 & 	$r^+$        	 & 	$K_S$    	 & 	$B_{J,878} V_{843} R_{C,844} I_{C,879}$                                  	 & 	LC2,CLASH-WL,WtG               	 & 	--               	\\
PSZ2 G205.93-39.46	 & 	$V_J R_C I_C$              	 & 	--             	 & 	$r$ 	 & 	$r^+$        	 & 	$K_S$    	 & 	--                                                                       	 & 	LC2,WtG                        	 & 	--               	\\
PSZ2 G056.93-55.08	 & 	$B_J V_J R_C I_C z^+$      	 & 	--             	 & 	$u g r i$ 	 & 	$r^+ i^+$    	 & 	--       	 & 	--                                                                       	 & 	LC2,WtG                        	 & 	--               	\\
PSZ2 G324.04+48.79	 & 	$V_J R_C I_C z^+$          	 & 	--             	 & 	$u g r i$ 	 & 	$r^+$        	 & 	$K_S$    	 & 	$B_{J,878} V_{843} R_{C,844} I_{C,879}$                                  	 & 	LC2,CLASH-WL,WtG,CCCP100       	 & 	--               	\\
PSZ2 G210.64+17.09	 & 	--                         	 & 	--             	 & 	$r$ 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	--               	\\
PSZ2 G044.77-51.30	 & 	$B_J V_J R_C I_C z^+$      	 & 	--             	 & 	$u r$ 	 & 	$r^+$        	 & 	$J H$    	 & 	--                                                                       	 & 	LC2,WtG                        	 & 	--               	\\
PSZ2 G201.50-27.31	 & 	$B_J V_J R_C i^+ I_C z^+$  	 & 	--             	 & 	$u g r i$ 	 & 	$r^+$        	 & 	$J K_S H$	 & 	--                                                                       	 & 	LC2,WtG,CCCP100                	 & 	--               	\\
PSZ2 G004.45-19.55	 & 	--                         	 & 	--             	 & 	 -- 	 & 	$i^+$        	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	--               	\\
PSZ2 G228.16+75.20	 & 	$B_J V_J R_C i^+ I_C z^+$  	 & 	$z^+$          	 & 	$u r$ 	 & 	--           	 & 	$K_S$    	 & 	--                                                                       	 & 	LC2,CLASH-WL,WtG               	 & 	--               	\\
PSZ2 G111.61-45.71	 & 	$B_J V_J R_C I_C$          	 & 	$r^+ i^+ z^+ Y$	 & 	$u g r i$ 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	LC2,WtG,CCCP100                	 & 	--               	\\
PSZ2 G155.27-68.42	 & 	--                         	 & 	$r^+ i^+$      	 & 	$u g r i$ 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	DES              	\\
PSZ2 G066.41+27.03	 & 	$i^+$                      	 & 	--             	 & 	 -- 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	CFIS             	\\
PSZ2 G339.63-69.34	 & 	--                         	 & 	--             	 & 	 -- 	 & 	--           	 & 	--       	 & 	--                                                                       	 & 	--                             	 & 	DES              	\\

